HOC-Search: Efficient CAD Model and Pose Retrieval from RGB-D Scans

We present an automated and efficient approach for retrieving high-quality CAD models of objects and their poses in a scene captured by a moving RGB-D camera. We first investigate various objective functions to measure similarity between a candidate CAD object model and the available data, and the best objective function appears to be a "render-and-compare" method comparing depth and mask rendering. We thus introduce a fast-search method that approximates an exhaustive search based on this objective function for simultaneously retrieving the object category, a CAD model, and the pose of an object given an approximate 3D bounding box. This method involves a search tree that organizes the CAD models and object properties including object category and pose for fast retrieval and an algorithm inspired by Monte Carlo Tree Search, that efficiently searches this tree. We show that this method retrieves CAD models that fit the real objects very well, with a speed-up factor of 10x to 120x compared to exhaustive search.

==> 4_0Top5Figure.tex <==
%\newcommand{\widthtopf}{0.07}
\newcommand{\widthtopf}{0.16}

\begin{figure}
\centering
%\scalebox{0.85}{
\scalebox{0.62}{
\begin{tabular}{c|ccc|ccc}
%[trim={left bottom right top}
  
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/scan.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/exh1.png} &  
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/exh2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/exh3.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0025_01_8_bookshelf/exh4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0025_01_8_bookshelf/exh5.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/mcts1.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/mcts2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0025_01_8_bookshelf/mcts3.png}
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0025_01_8_bookshelf/mcts4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0025_01_8_bookshelf/mcts5.png}
  \\


    \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/scan.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/exh1.png} &  
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/exh2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/exh3.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0030_00_4_sofa/exh4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0030_00_4_sofa/exh5.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/mcts1.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/mcts2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0030_00_4_sofa/mcts3.png}
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0030_00_4_sofa/mcts4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0030_00_4_sofa/mcts5.png} 
  \\

  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/scan.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/exh1.png} &  
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/exh2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/exh3.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0575_00_4_chair/exh4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0575_00_4_chair/exh5.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/mcts1.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/mcts2.png} &
  \includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0575_00_4_chair/mcts3.png}
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0575_00_4_chair/mcts4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 5.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0575_00_4_chair/mcts5.png} 
  \\
%[trim={left bottom right top}

   \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/scan.png} &
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/exh1.png} &  
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/exh2.png} &
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/exh3.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 6.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0000_00_0_bed/exh4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 6.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0000_00_0_bed/exh5.png} &
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/mcts1.png} &
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/mcts2.png} &
  \includegraphics[trim={11cm 2.5cm 13cm 7.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results_v2/scene0144_00_3_bed/mcts3.png} 
  %\includegraphics[trim={15cm 2.5cm 15cm 6.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0000_00_0_bed/mcts4.png} &
  %\includegraphics[trim={15cm 2.5cm 15cm 6.cm},clip,width=\widthtopf\linewidth]{figures/comparison_top5_results/scene0000_00_0_bed/mcts5.png} 
  \\
  Target object & 
  \multicolumn{3}{c|}{Top-3 candidates, exhaustive search} &
  \multicolumn{3}{c}{Top-3 candidates, HOC-Search (ours)} \\  
  % object & &&&& & &&&&\\
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Visualization of top-3 candidates (in descending order) from exhaustive search compared to HOC-Search for 800 iterations. Left shows the target object, middle column are the results from the exhaustive search, and right column shows the results using our HOC-Search. Although not always the same model is found, the overall quality of HOC-Search is very high. The two methods retrieve very similar CAD models.
We refer to the supplementary material for additional visualizations.
}
    \label{fig:vis_topk_acc}
\end{figure}

==> supp_unknown_catFigure.tex <==

\definecolor{chair_color}{rgb}{0.301, 0.745, 0.933}
\definecolor{cabinet_color}{rgb}{0.494, 0.184, 0.556}
\definecolor{bed_color}{rgb}{0.466, 0.674, 0.188}
\definecolor{sofa_color}{rgb}{0.635, 0.078, 0.184}
\definecolor{table_color}{rgb}{0.000, 0.667, 0.000}
\definecolor{bookshelf_color}{rgb}{0.000, 0.000, 1.000}
\definecolor{lamp_color}{rgb}{1.000, 0.333, 0.500}
\definecolor{display_color}{rgb}{0.333, 0.667, 1.000}


\begin{figure*}
\centering
\scalebox{0.85}{
\begin{tabular}{cccc}
%[trim={left bottom right top}
% \includegraphics[trim={2cm 4cm 4cm 3cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0549_01/scene_boxes.png} &
%  \includegraphics[trim={2cm 4cm 4cm 3cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0549_01/exh_search.png} &
%  \includegraphics[trim={2cm 4cm 4cm 3cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0549_01/hoc_800.png} &
%  \includegraphics[trim={2cm 4cm 4cm 3cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0549_01/hoc_1200.png} \\

 \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/scene_boxes.png} &
  \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/exh_search.png} &
  \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/hoc_800.png} &
  \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/hoc_1200.png} \\

%   \includegraphics[trim={7cm 3cm 7cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0435_00/scene_boxes.png} &
%  \includegraphics[trim={7cm 3cm 7cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0435_00/exh_search.png} &
%  \includegraphics[trim={7cm 3cm 7cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0435_00/hoc_800.png} &
%  \includegraphics[trim={7cm 3cm 7cm 4cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0435_00/hoc_1200.png} \\

%   \includegraphics[trim={8cm 4cm 8cm 4.5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0609_01/scene_boxes.png} &
%  \includegraphics[trim={8cm 4cm 8cm 4.5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0609_01/exh_search.png} &
%  \includegraphics[trim={8cm 4cm 8cm 4.5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0609_01/hoc_800.png} &
%  \includegraphics[trim={8cm 4cm 8cm 4.5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0609_01/hoc_1200.png} \\

     \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/scene_boxes.png} &
  \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/exh_search.png} &
  \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/hoc_800.png} &
  \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/hoc_1200.png} \\

%     \includegraphics[trim={6cm 1cm 11cm 6cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0690_01/scene_boxes.png} &
%  \includegraphics[trim={6cm 1cm 11cm 6cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0690_01/exh_search.png} &
%  \includegraphics[trim={6cm 1cm 11cm 6cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0690_01/hoc_800.png} &
%  \includegraphics[trim={6cm 1cm 11cm 6cm},clip,width=0.25\linewidth]{figures/results_HOC_unknown_cat/scene0690_01/hoc_1200.png} \\
  
  RGB-D Scan with &  Results using exh. search & HOC-Search (800 iterations)  &HOC-Search (1200 iterations) \\
   initial 3D boxes         &   \textbf{with category label}   &      without category label    & without category label\\
\end{tabular}
}
\caption{
\stefan{
Qualitative results for CAD model and pose retrieval for objects with unknown category label.
From left to right, we show 1) the input scan with initial 3D boxes, 2) the CAD models retrieved with exhaustive search \textbf{and} ground-truth category label as reference result, and 3) - 4) the results of HOC-Search for unknown category labels for 800 and 1200 iterations, respectively. Although the complexity for retrieval highly increases with unknown category labels, HOC-Search is able to find suitable CAD models and predict the correct object poses. Note that HOC-Search does not always retrieve the same category label as in the ground-truth, however, this is mainly due to ambiguities of category labels (e.g. the categories Chair and Sofa share very similar CAD models, the same applies to Bookshelf and Cabinet). The color of the retrieved objects refers to the category label: \textcolor{chair_color}{Chair}, \textcolor{cabinet_color}{Cabinet}, \textcolor{bed_color}{Bed}, \textcolor{sofa_color}{Sofa}, \textcolor{table_color}{Table}, \textcolor{bookshelf_color}{Bookshelf}, \textcolor{lamp_color}{Lamp}, \textcolor{display_color}{Display}.
}
}
\label{fig:supp_unknown_cat}
\end{figure*}

==> supp_unknown_catFigure_v2.tex <==

\definecolor{chair_color}{rgb}{0.301, 0.745, 0.933}
\definecolor{cabinet_color}{rgb}{0.494, 0.184, 0.556}
\definecolor{bed_color}{rgb}{0.466, 0.674, 0.188}
\definecolor{sofa_color}{rgb}{0.635, 0.078, 0.184}
\definecolor{table_color}{rgb}{0.000, 0.667, 0.000}
\definecolor{bookshelf_color}{rgb}{0.000, 0.000, 1.000}
\definecolor{lamp_color}{rgb}{1.000, 0.333, 0.500}
\definecolor{display_color}{rgb}{0.333, 0.667, 1.000}


\begin{figure}
\centering
\scalebox{0.85}{
\begin{tabular}{cc}
%[trim={left bottom right top}

 \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/scene_boxes.png} &
      \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/scene_boxes.png} \\
  \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/exh_search.png} &
  \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/exh_search.png} \\
  \includegraphics[trim={7cm 3cm 8cm 4cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0030_00/hoc_800.png} &
    \includegraphics[trim={8cm 4cm 10cm 5cm},clip,width=0.5\linewidth]{figures/results_HOC_unknown_cat/scene0616_01/hoc_800.png} \\
\end{tabular}
}
\caption{
\stefan{
Qualitative results for CAD model and pose retrieval for objects with unknown category label.
From left to right, we show 1) the input scan with initial 3D boxes, 2) the CAD models retrieved with exhaustive search \textbf{and} ground-truth category label as reference result, and 3) the results of HOC-Search for unknown category labels for 800 iterations. Although the complexity for retrieval highly increases with unknown category labels, HOC-Search is able to find suitable CAD models and predict the correct object poses. Note that HOC-Search does not always retrieve the same category label as in the ground-truth, however, this is mainly due to ambiguities of category labels (e.g. the categories Chair and Sofa share very similar CAD models, the same applies to Bookshelf and Cabinet). The color of the retrieved objects refers to the category label: \textcolor{chair_color}{Chair}, \textcolor{cabinet_color}{Cabinet}, \textcolor{bed_color}{Bed}, \textcolor{sofa_color}{Sofa}, \textcolor{table_color}{Table}, \textcolor{bookshelf_color}{Bookshelf}, \textcolor{lamp_color}{Lamp}, \textcolor{display_color}{Display}.
}
}
\label{fig:supp_unknown_cat_v2}
\end{figure}
